It Takes (Only) Two: Adversarial Generator-Encoder Networks

We present a new autoencoder-type architecture that is trainable in an unsupervised mode, sustains both generation and inference, and has the quality of conditional and unconditional samples boosted by adversarial learning. Unlike previous hybrids of autoencoders and adversarial networks, the adversarial game in our approach is set up directly between the encoder and the generator, and no external mappings are trained in the process of learning. The game objective compares the divergences of each of the real and the generated data distributions with the prior distribution in the latent space. We show that direct generator-vs-encoder game leads to a tight coupling of the two components, resulting in samples and reconstructions of a comparable quality to some recently-proposed more complex architectures.

==> related.tex <==
\section{Related work}

As discussed in the introduction, joint learning of inference and generation is a hot topic of research. The methods that combine adversarial training with such simultaneous training, include approaches adversarially learned inference (adversarial feature learning)~ \cite{Dumoulin16,Donahue16}, the approach~\cite{Larsen15}, and adversarial autoencoders~\cite{Makhzani15}. Arguably, our approach has more similarity with~\cite{Dumoulin16,Donahue16}, as in their case, the alignment involves the latent space distribution, and the generators are also involved into the adversarial learning game. Also, \cite{Dumoulin16} provides most extensive evaluation for the image sampling and reconstruction process, hence we make their method our main reference for comparisons. 

Perhaps, the main novelty of our architecture is the new game objective for adversarial learning that is computed at batch level (rather than for individual samples). Recently, \cite{Salimans16} proposed to use batch-level information for adversarial training was first proposed in to prevent mode collapse. Their discriminator still performs individual sample classification, but admixes the descriptor based on distances to other samples in the batch into the individual sample feature descriptor. Interestingly, our method can also uses pairwise distances in a batch for the estimation of the divergences.

Another avenue for improving the stability of GANs is the replacement of the classifying discriminator with the regression-based one as in energy-based GANs~\cite{Zhao16} and Wasserstein GANs~\cite{Arjovsky17}. Our statistics (the divergence from the canonical distribution) can be seen as a very special form of regression. In this way, the encoder in our architecture can be seen as a discriminator computing a single number similarly to how it is done in \cite{Zhao16,Arjovsky17}.


